On Feature Importance and Interpretability of Speaker Representations

Unsupervised speech disentanglement aims at separating fast varying from slowly varying components of a speech signal. In this contribution, we take a closer look at the embedding vector representing the slowly varying signal components, commonly named the speaker embedding vector. We ask, which properties of a speaker's voice are captured and investigate to which extent do individual embedding vector components sign responsible for them, using the concept of Shapley values. Our findings show that certain speaker-specific acoustic-phonetic properties can be fairly well predicted from the speaker embedding, while the investigated more abstract voice quality features cannot.

==> manipulation_example.tex <==
% This file was created with tikzplotlib v0.10.1.
\pgfplotsset{
compat=1.11,
legend image code/.code={
\draw[mark repeat=2,mark phase=2]
plot coordinates {
(0cm,0cm)
(0.15cm,0cm)        %% default is (0.3cm,0cm)
(0.45cm,0cm)         %% default is (0.6cm,0cm)
};%
}
}

\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{sienna1409760}{RGB}{140,97,60}

\begin{groupplot}[group style={group size=1 by 2, vertical sep=0.5cm}]
\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.2,-0.1)}, draw=lightgray204},
scaled x ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={},
xmajorgrids,
xmin=-14, xmax=14,
xtick style={color=black},
xticklabels={},
y grid style={darkgray176},
ylabel={\(\displaystyle \hat{y}_{\mathrm{p}}\)},
ymajorgrids,
ymin=10, ymax=50,
ytick style={color=black},
height=3cm,
width=8cm,
ylabel style = {at={(-0.1, 0.5)}},
]
\addplot [very thick, steelblue31119180]
table {%
-14 18.0769195556641
-12 16.7729644775391
-10 20.1262283325195
-8 29.5510673522949
-6 29.7776489257812
-4 29.2460269927979
-2 31.1415824890137
0 36.2064208984375
2 37.0504875183105
4 37.6751861572266
6 40.9540252685547
8 45.7695350646973
10 46.71044921875
12 46.7252655029297
14 46.6458206176758
};

\addplot [ultra thick, dotted, darkorange25512714]
table {%
-14 33.538646697998
-12 18.6517143249512
-10 16.9934730529785
-8 17.8149433135986
-6 29.5585041046143
-4 29.8761234283447
-2 28.8871231079102
0 25.1726703643799
2 32.7304420471191
4 35.7461318969727
6 36.8966751098633
8 41.6745758056641
10 46.3208160400391
12 46.8968315124512
14 46.8088912963867
};
\addplot[domain=-14:14, dashed, very thick, black] {26};
\addplot[domain=-14:14, dashed, very thick, red] {36};
\nextgroupplot[
legend cell align={left},
legend style={at={(1.05,-0.6)}, draw=lightgray204, legend columns=5},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle \gamma\)},
xlabel style={, at={(0.5,-0.3)}},
xmajorgrids,
xmin=-14, xmax=14,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\(\displaystyle \hat{y}_\mathrm{h}\)},
ylabel style = {at={(-0.1, 0.5)}},
ymajorgrids,
ymin=15, ymax=40,
ytick style={color=black},
height=3cm,
width=8cm,
]
\addlegendimage{ultra thick, dotted, darkorange25512714}
\addlegendentry{$\hat{y}_\mathrm{p, male}$}
\addlegendimage{very thick, steelblue31119180}
\addlegendentry{$\hat{y}_\mathrm{p, female}$ }
\addlegendimage{very thick, black, dashed}
\addlegendentry{$\bar{y}_\mathrm{p, male}$}
\addlegendimage{very thick, red, dashed}
\addlegendentry{$\bar{y}_\mathrm{p, female}$}
\addplot [very thick, sienna1409760]
table {%
-14 18.6672954559326
-12 19.3840789794922
-10 20.3438205718994
-8 21.4520244598389
-6 22.7084579467773
-4 24.1310691833496
-2 25.5638160705566
0 27.0076198577881
2 28.4772262573242
4 29.9624919891357
6 31.4655075073242
8 33.0242156982422
10 34.5591583251953
12 36.0835952758789
14 37.5786018371582
};
\addlegendentry{$\hat{y}_\mathrm{h}$}
\end{groupplot}

\end{tikzpicture}


==> manipulation_gender_one_component.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{sienna1409760}{RGB}{140,97,60}

\begin{groupplot}[group style={group size=1 by 2, vertical sep=0.65cm}]
\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.91,0.5)},
  anchor=east,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={},
xmajorgrids,
xmin=-6.6, xmax=6.6,
xtick style={color=black},
xticklabels={},
y grid style={darkgray176},
ylabel={Accuracy [\(\displaystyle \%\)]},
ymajorgrids,
ymin=-5, ymax=105,
ytick style={color=black},
height=3cm,
width=8.5cm,
]
\addplot [very thick, darkgray176]
table {%
-6 100
-4 100
-2 100
0 100
2 14.4444444444444
4 0
6 0
};
\addplot [ultra thick, dotted, darkorange25512714]
table {%
-6 0
-4 0
-2 32.7272727272727
0 98.1818181818182
2 100
4 100
6 100
};
\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.91,0.5)},
  anchor=east,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Index $\gamma$},
xmajorgrids,
xmin=-6.6, xmax=6.6,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Accuracy [\(\displaystyle \%\)]},
ymajorgrids,
ymin=-5, ymax=105,
ytick style={color=black},
height=3cm,
width=8.5cm,
legend cell align={left},
legend style={at={(1,-1)}, draw=lightgray204, legend columns=5},
]
\addlegendentry{male}
\addlegendimage{very thick, darkgray176}
\addlegendentry{female}
\addlegendimage{ultra thick, dotted, darkorange25512714}

\addplot [very thick, steelblue31119180]
table {%
-6 96.078431372549
-4 94.1176470588235
-2 91.1764705882353
0 79.4117647058823
2 58.8235294117647
4 50
6 46.078431372549
};
\addlegendentry{not nasal}
\addplot [ultra thick, dotted, sienna1409760]
table {%
-6 8.16326530612245
-4 20.4081632653061
-2 37.7551020408163
0 56.1224489795918
2 63.265306122449
4 69.3877551020408
6 68.3673469387755
};
\addlegendentry{nasal}
\end{groupplot}
\end{tikzpicture}



==> shapley_values_gender.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
title={Gender},
x grid style={darkgray176},
%xlabel={Component \(\displaystyle i\)},
xticklabels={},
xmajorgrids,
xmin=0, xmax=64,
xtick style={color=black},
y grid style={darkgray176},
ylabel={$\nicefrac{|\phi_{\mathrm{g}, i}|}{|| \boldsymbol{\phi}_{\mathrm{g}} ||}$},
ymajorgrids,
ymin=0, ymax=0.4,
ytick style={color=black},
width=8.5cm,
height=3cm,
%ytick={0.05, 0.1,0.4},
xlabel={Component \(\displaystyle i\)},
%yticklabels={0.05, 0.1,0.15},
y label style={at={(axis description cs:-0.02,0.5)},anchor=north},
]
\path [draw=steelblue31119180, semithick]
(axis cs:0,0)
--(axis cs:0,0.0022079928831811);

\path [draw=steelblue31119180, semithick]
(axis cs:1,0)
--(axis cs:1,0.0644247256309603);

\path [draw=steelblue31119180, semithick]
(axis cs:2,0)
--(axis cs:2,0.0696777230489745);

\path [draw=steelblue31119180, semithick]
(axis cs:3,0)
--(axis cs:3,0.00599649712152813);

\path [draw=steelblue31119180, semithick]
(axis cs:4,0)
--(axis cs:4,0.0012548442510604);

\path [draw=steelblue31119180, semithick]
(axis cs:5,0)
--(axis cs:5,0.00374725416996564);

\path [draw=steelblue31119180, semithick]
(axis cs:6,0)
--(axis cs:6,0.00727787423972211);

\path [draw=steelblue31119180, semithick]
(axis cs:7,0)
--(axis cs:7,0.000662312669498822);

\path [draw=steelblue31119180, semithick]
(axis cs:8,0)
--(axis cs:8,0.074394996842317);

\path [draw=steelblue31119180, semithick]
(axis cs:9,0)
--(axis cs:9,1.31892312582453e-05);

\path [draw=steelblue31119180, semithick]
(axis cs:10,0)
--(axis cs:10,0.00495217524179494);

\path [draw=steelblue31119180, semithick]
(axis cs:11,0)
--(axis cs:11,0.00542145376360318);

\path [draw=steelblue31119180, semithick]
(axis cs:12,0)
--(axis cs:12,0.00110476441735455);

\path [draw=steelblue31119180, semithick]
(axis cs:13,0)
--(axis cs:13,0.00183423166976545);

\path [draw=steelblue31119180, semithick]
(axis cs:14,0)
--(axis cs:14,0.0165872444888041);

\path [draw=steelblue31119180, semithick]
(axis cs:15,0)
--(axis cs:15,0.0790966598953228);

\path [draw=steelblue31119180, semithick]
(axis cs:16,0)
--(axis cs:16,0.00537017188407852);

\path [draw=steelblue31119180, semithick]
(axis cs:17,0)
--(axis cs:17,0.0038403380718776);

\path [draw=steelblue31119180, semithick]
(axis cs:18,0)
--(axis cs:18,0.00276525221070728);

\path [draw=steelblue31119180, semithick]
(axis cs:19,0)
--(axis cs:19,0.317318586598456);

\path [draw=steelblue31119180, semithick]
(axis cs:20,0)
--(axis cs:20,0.00513767103570739);

\path [draw=steelblue31119180, semithick]
(axis cs:21,0)
--(axis cs:21,0.0168354234540473);

\path [draw=steelblue31119180, semithick]
(axis cs:22,0)
--(axis cs:22,0.00130883240253177);

\path [draw=steelblue31119180, semithick]
(axis cs:23,0)
--(axis cs:23,0.0188918133227609);

\path [draw=steelblue31119180, semithick]
(axis cs:24,0)
--(axis cs:24,0.000766164191375471);

\path [draw=steelblue31119180, semithick]
(axis cs:25,0)
--(axis cs:25,0.000722666121804548);

\path [draw=steelblue31119180, semithick]
(axis cs:26,0)
--(axis cs:26,0.00854964959567536);

\path [draw=steelblue31119180, semithick]
(axis cs:27,0)
--(axis cs:27,0.00175310813375639);

\path [draw=steelblue31119180, semithick]
(axis cs:28,0)
--(axis cs:28,0.00304170772581836);

\path [draw=steelblue31119180, semithick]
(axis cs:29,0)
--(axis cs:29,0.00207004946895372);

\path [draw=steelblue31119180, semithick]
(axis cs:30,0)
--(axis cs:30,0.00381368389009501);

\path [draw=steelblue31119180, semithick]
(axis cs:31,0)
--(axis cs:31,0.0013081371168218);

\path [draw=steelblue31119180, semithick]
(axis cs:32,0)
--(axis cs:32,0.00516278784845523);

\path [draw=steelblue31119180, semithick]
(axis cs:33,0)
--(axis cs:33,0.00211718668211581);

\path [draw=steelblue31119180, semithick]
(axis cs:34,0)
--(axis cs:34,0.0015558745262145);

\path [draw=steelblue31119180, semithick]
(axis cs:35,0)
--(axis cs:35,0.000326811145974223);

\path [draw=steelblue31119180, semithick]
(axis cs:36,0)
--(axis cs:36,0.00553494807747783);

\path [draw=steelblue31119180, semithick]
(axis cs:37,0)
--(axis cs:37,0.000391903173402472);

\path [draw=steelblue31119180, semithick]
(axis cs:38,0)
--(axis cs:38,0.00147735692314412);

\path [draw=steelblue31119180, semithick]
(axis cs:39,0)
--(axis cs:39,0.0001848550606558);

\path [draw=steelblue31119180, semithick]
(axis cs:40,0)
--(axis cs:40,0.00319423079544683);

\path [draw=steelblue31119180, semithick]
(axis cs:41,0)
--(axis cs:41,0.0104191469467992);

\path [draw=steelblue31119180, semithick]
(axis cs:42,0)
--(axis cs:42,0.00347745866102852);

\path [draw=steelblue31119180, semithick]
(axis cs:43,0)
--(axis cs:43,0.000427398968815719);

\path [draw=steelblue31119180, semithick]
(axis cs:44,0)
--(axis cs:44,0.0023152383026408);

\path [draw=steelblue31119180, semithick]
(axis cs:45,0)
--(axis cs:45,0.00196558209826526);

\path [draw=steelblue31119180, semithick]
(axis cs:46,0)
--(axis cs:46,0.00331772165004361);

\path [draw=steelblue31119180, semithick]
(axis cs:47,0)
--(axis cs:47,0.00176467265762493);

\path [draw=steelblue31119180, semithick]
(axis cs:48,0)
--(axis cs:48,0.00549523758867157);

\path [draw=steelblue31119180, semithick]
(axis cs:49,0)
--(axis cs:49,0.00179114535468787);

\path [draw=steelblue31119180, semithick]
(axis cs:50,0)
--(axis cs:50,0.000210909294655532);

\path [draw=steelblue31119180, semithick]
(axis cs:51,0)
--(axis cs:51,0.00232446248034615);

\path [draw=steelblue31119180, semithick]
(axis cs:52,0)
--(axis cs:52,0.00145127100848425);

\path [draw=steelblue31119180, semithick]
(axis cs:53,0)
--(axis cs:53,0.00151447373441333);

\path [draw=steelblue31119180, semithick]
(axis cs:54,0)
--(axis cs:54,0.00286133012516622);

\path [draw=steelblue31119180, semithick]
(axis cs:55,0)
--(axis cs:55,0.00501413657633647);

\path [draw=steelblue31119180, semithick]
(axis cs:56,0)
--(axis cs:56,0.0151070202081494);

\path [draw=steelblue31119180, semithick]
(axis cs:57,0)
--(axis cs:57,0.0037968853474956);

\path [draw=steelblue31119180, semithick]
(axis cs:58,0)
--(axis cs:58,0.000180881473115549);

\path [draw=steelblue31119180, semithick]
(axis cs:59,0)
--(axis cs:59,0.00662186739668697);

\path [draw=steelblue31119180, semithick]
(axis cs:60,0)
--(axis cs:60,0.0141412463786056);

\path [draw=steelblue31119180, semithick]
(axis cs:61,0)
--(axis cs:61,0.00128142670549197);

\path [draw=steelblue31119180, semithick]
(axis cs:62,0)
--(axis cs:62,0.0151584319841633);

\path [draw=steelblue31119180, semithick]
(axis cs:63,0)
--(axis cs:63,0.147268906035847);

\addplot [semithick, steelblue31119180, mark=*, mark size=1, mark options={solid}, only marks]
table {%
0 0.0022079928831811
1 0.0644247256309603
2 0.0696777230489745
3 0.00599649712152813
4 0.0012548442510604
5 0.00374725416996564
6 0.00727787423972211
7 0.000662312669498822
8 0.074394996842317
9 1.31892312582453e-05
10 0.00495217524179494
11 0.00542145376360318
12 0.00110476441735455
13 0.00183423166976545
14 0.0165872444888041
15 0.0790966598953228
16 0.00537017188407852
17 0.0038403380718776
18 0.00276525221070728
19 0.317318586598456
20 0.00513767103570739
21 0.0168354234540473
22 0.00130883240253177
23 0.0188918133227609
24 0.000766164191375471
25 0.000722666121804548
26 0.00854964959567536
27 0.00175310813375639
28 0.00304170772581836
29 0.00207004946895372
30 0.00381368389009501
31 0.0013081371168218
32 0.00516278784845523
33 0.00211718668211581
34 0.0015558745262145
35 0.000326811145974223
36 0.00553494807747783
37 0.000391903173402472
38 0.00147735692314412
39 0.0001848550606558
40 0.00319423079544683
41 0.0104191469467992
42 0.00347745866102852
43 0.000427398968815719
44 0.0023152383026408
45 0.00196558209826526
46 0.00331772165004361
47 0.00176467265762493
48 0.00549523758867157
49 0.00179114535468787
50 0.000210909294655532
51 0.00232446248034615
52 0.00145127100848425
53 0.00151447373441333
54 0.00286133012516622
55 0.00501413657633647
56 0.0151070202081494
57 0.0037968853474956
58 0.000180881473115549
59 0.00662186739668697
60 0.0141412463786056
61 0.00128142670549197
62 0.0151584319841633
63 0.147268906035847
};
\end{axis}

\end{tikzpicture}

